Instance Semantic Segmentation Benefits from Generative Adversarial Networks

In design of instance segmentation networks that reconstruct masks, segmentation is often taken as its literal definition -- assigning each pixel a label. This has led to thinking the problem as a template matching one with the goal of minimizing the loss between the reconstructed and the ground truth pixels. Rethinking reconstruction networks as a generator, we define the problem of predicting masks as a GANs game framework: A segmentation network generates the masks, and a discriminator network decides on the quality of the masks. To demonstrate this game, we show effective modifications on the general segmentation framework in Mask R-CNN. We find that playing the game in feature space is more effective than the pixel space leading to stable training between the discriminator and the generator, predicting object coordinates should be replaced by predicting contextual regions for objects, and overall the adversarial loss helps the performance and removes the need for any custom settings per different data domain. We test our framework in various domains and report on cellphone recycling, autonomous driving, large-scale object detection, and medical glands. We observe in general GANs yield masks that account for crispier boundaries, clutter, small objects, and details, being in domain of regular shapes or heterogeneous and coalescing shapes. Our code for reproducing the results is available publicly.

==> table/coco_acc.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
% \usepackage{graphicx}
\begin{table}[!htb]
\centering
\caption{The 2017 COCO object detection (A) and segmentation (B) results (bounding box and mask AP). Comparisons between the baseline Mask-RCNN and our model on the \textit{validation} set. ResNet-101-FPN is used in both cases. Our model using GAN framework achieves comparable performance in bounding box AP and 0.8$\%$ improvement in mask AP metric compared to Mask-RCNN.}
\resizebox{\columnwidth}{!}{%
\begin{tabular}{c|c|ccc|ccc}
                   &       & $AP$            & $AP_{50}$       & $AP_{75}$       & $AP_{S}$        & $AP_{M}$        & $AP_{L}$        \\ \hline
\multirow{2}{*}{A} & MRCNN & 0.3992          & 0.6116          & \textbf{0.4387} & \textbf{0.2336} & 0.4328          & 0.5183          \\
                   & Ours  & \textbf{0.3994} & \textbf{0.6143} & 0.4342          & 0.2317          & \textbf{0.4332} & \textbf{0.5269} \\ \hline
\multirow{2}{*}{B} & MRCNN & 0.3604          & 0.5828          & 0.3835          & 0.1606          & 0.3892          & 0.5299          \\
 & Ours & \textbf{0.3681} & \textbf{0.5855} & \textbf{0.3919} & \textbf{0.1685} & \textbf{0.3988} & \textbf{0.5452}
\end{tabular}%
}
\label{tab:coco_acc}
\end{table}

==> table/gland_acc.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
% \usepackage{graphicx}
\begin{table}[!htb]
\centering
\caption{The MICCAI 2015 medical gland (A) and segmentation (B) results (bounding box and mask AP). Comparisons between the baseline Mask-RCNN and our model on the Gland \textit{test} set. ResNet-50-FPN is used in both cases. Our model using GAN framework achieves $1.7\%$ and 2.7$\%$ improvement in bounding box and mask AP metric respectively compared to Mask-RCNN.}
\resizebox{\columnwidth}{!}{%
\begin{tabular}{c|c|ccc|cc}
                   &       & $AP$            & $AP_{50}$       & $AP_{75}$       & $AP_{M}$        & $AP_{L}$        \\ \hline
\multirow{2}{*}{A} & MRCNN & 0.5689          & 0.8174          & 0.6419          & 0.5940          & 0.5717          \\
                   & Ours  & \textbf{0.5855} & \textbf{0.8398} & \textbf{0.6668} & \textbf{0.6057} & \textbf{0.5983} \\ \hline
\multirow{2}{*}{B} & MRCNN & 0.5892          & 0.8014          & 0.9814          & 0.589           & 0.6189          \\
                   & Ours  & \textbf{0.6156} & \textbf{0.8236} & \textbf{0.7054} & \textbf{0.6054} & \textbf{0.6516}
\end{tabular}%
}
\label{tab:gland_acc}
\end{table}

==> table/phone_acc.tex <==

\begin{table}[!htb]
\centering
\caption{Phone recycling object detection (A) and segmentation (B) results (bounding box and mask AP). Comparisons between the baseline Mask-RCNN and our model on the Phone Recycling \textit{validation} set. ResNet-101-FPN is used in both cases. Our model using GAN framework achieves $3.6\%$ and 2.1$\%$ improvement in bounding box and mask AP respectively compared to Mask-RCNN.}
\resizebox{\columnwidth}{!}{%
\begin{tabular}{c|c|ccc|ccc}
                   &       & $AP$            & $AP_{50}$       & $AP_{75}$       & $AP_{S}$        & $AP_{M}$        & $AP_{L}$        \\ \hline
\multirow{2}{*}{A} & MRCNN & 0.5486          & 0.7333          & 0.6261          & 0.3327          & 0.5071          & 0.7462          \\
                   & Ours  & \textbf{0.5844} & \textbf{0.7746} & \textbf{0.6448} & \textbf{0.3833} & \textbf{0.5480} & \textbf{0.7586} \\ \hline
\multirow{2}{*}{B} & MRCNN & 0.5718          & 0.7242          & 0.6439          & 0.3195          & 0.5247          & 0.7735          \\
                   & Ours  & \textbf{0.5923} & \textbf{0.7607} & \textbf{0.6525} & \textbf{0.3615} & \textbf{0.5549} & \textbf{0.7846}
\end{tabular}%
}
\label{tab:phone_acc}
\end{table}
